Tight complexity lower bounds for integer linear programming with few constraints

We consider the ILP Feasibility problem: given an integer linear program $\{Ax = b, x\geq 0\}$, where $A$ is an integer matrix with $k$ rows and $\ell$ columns and $b$ is a vector of $k$ integers, we ask whether there exists $x\in\mathbb{N}^\ell$ that satisfies $Ax = b$. Our goal is to study the complexity of ILP Feasibility when both $k$, the number of constraints (rows of $A$), and $\|A\|_\infty$, the largest absolute value in $A$, are small. Papadimitriou [J. ACM, 1981] was the first to give a fixed-parameter algorithm for ILP Feasibility in this setting, with running time $\left((\|A\mid b\|_\infty) \cdot k\right)^{O(k^2)}$. This was very recently improved by Eisenbrand and Weismantel [SODA 2018], who used the Steinitz lemma to design an algorithm with running time $(k\|A\|_\infty)^{O(k)}\cdot \|b\|_\infty^2$, and subsequently by Jansen and Rohwedder [2018] to $O(k\|A\|_\infty)^{k}\cdot \log \|b\|_\infty$. We prove that for $\{0,1\}$-matrices $A$, the dependency on $k$ is probably optimal: an algorithm with running time $2^{o(k\log k)}\cdot (\ell+\|b\|_\infty)^{o(k)}$ would contradict ETH. This improves previous non-tight lower bounds of Fomin et al. [ESA 2018]. We then consider ILPs with many constraints, but structured in a shallow way. Precisely, we consider the dual treedepth of the matrix $A$, which is the treedepth of the graph over the rows of $A$, with two rows adjacent if in some column they both contain a non-zero entry. It was recently shown by Kouteck\'{y} et al. [ICALP 2018] that ILP Feasibility can be solved in time $\|A\|_\infty^{2^{O(td(A))}}\cdot (k+\ell+\log \|b\|_\infty)^{O(1)}$. We present a streamlined proof of this fact and prove optimality: even assuming that all entries of $A$ and $b$ are in $\{-1,0,1\}$, the existence of an algorithm with running time $2^{2^{o(td(A))}}\cdot (k+\ell)^{O(1)}$ would contradict ETH.

==> bnd-support.tex <==

\section{Few constraints -- bounded support}
Let $\supp(\vex)$ be the set of indices of coordinates on which $\vex$ is non-zero.
\begin{theorem}
	Let $A \in \ZZ^{m \times n}$, $\veb \in \ZZ^m$ and suppose $\|A\|_\infty \leq \Delta$. Then every solution of $\{\vex \in \ZZ^n \mid A\vex=\veb, \vex \geq 0\}$ with (containment-wise) minimal support satisfies $|\supp(\vex)|\leq \Oh(m \log \Delta)$.
\end{theorem}
\begin{proof}
Let $\vex$ be a solution with minimal support; among solutions with the same support choose $\vex$ to be the lexicographically smallest.
%Without loss of generality we can assume $\vex \geq 0$ (otherwise negate each negative entry together with the corresponding column of $A$).
Let $\alpha = c \lceil\lg (\Delta+1)\rceil$ for a universal constant $c\geq 2$ to be chosen later and set $h = \alpha m$.
We show that $|\supp(\vex)|< 2h$.

Suppose to the contrary that $|\supp(\vex)| \geq 2h$.
For a subset $I \subseteq [n]$ let $\ve{1}_I \in \{0,1\}^n$ be the vector with support $I$.
Consider the set of all such vectors whose support is a subset of $\supp(\vex)$ of size $h$: $X=\{\ve{1}_I \in \{0,1\}^n \mid I \subseteq \supp(\vex), |I|=h\}$.
Clearly $|X| \geq \binom{2h}{h}$.

Observe that if for any two vectors $\ve{x'},\ve{x''} \in X$ we have $A\ve{x'} = A\ve{x''}$, then both $\ve{x}-\ve{x'}+\ve{x''}$ and $\ve{x}-\ve{x''}+\ve{x'}$ are feasible solutions with support contained in $\supp(\vex)$.
Moreover, at least one of them has strictly smaller support or has the same support but is lexicographically smaller.
This would contradict our choice of $\vex$, hence $A\ve{x'} \neq A\ve{x''}$ for all $\ve{x'},\ve{x''} \in X$.

However, for any $\ve{x'} \in X$, the vector $A\ve{x'}$ is an $m$-dimensional integer vector with $\|Ax'\|_\infty \leq \Delta h$.
Hence $|X|$ is bounded by the number of such vectors, which is at most $(2\Delta h+1)^{m}$ (each coordinate is between $-\Delta h$ and $+\Delta h$).
In fact $\|\ve{x'}\|_1 \leq h$, hence $\|A\ve{x'}\|_1 \leq \Delta h$, which allows us to use a better bound:

\begin{claim} The number of vectors $\ve{y} \in \ZZ^m$ with $\|\ve{y}\|_1 \leq \Delta h$ is at most $2^m \binom{\Delta h +m}{m}$.
\end{claim}
\begin{proof} 
The number of non-negative such vectors with  $\|\ve{y}\|_1 = \Delta h$ equals $\binom{\Delta h + m - 1}{m - 1}$.
We can choose signs in $2^m$ ways.
To account for vectors with $\|\ve{y}\|_1 < \Delta h$, it suffices to introduce a dummy coordinate (with value equal to $\Delta h - \|\ve{y}\|_1$), increasing $m$ by one.
\cqed
\end{proof}

Hence $\binom{2 \alpha m}{\alpha m} = \binom{2h}{h} \leq |X| \leq 2^m \binom{\Delta h + m}{m} = 2^m \binom{(\Delta \alpha + 1) m}{m}$.
The following claim implies that this is not possible.


\begin{claim}
There is a constant $c>1$ such that for any $m,\Delta \geq 1$ and $\alpha = c \lceil \lg(\Delta+1)\rceil$, we have
 $\binom{2 \alpha m}{\alpha m} > 2^m \binom{(\Delta \alpha + 1) m}{m}$.
\end{claim}
\begin{proof}
On one hand, since $\binom{2p}{p} > 2^p $ for $p>1$, we have 
$\lg \binom{2 \alpha m}{\alpha m} > \alpha m$.

On the other hand, $\binom{p}{\eps p} \leq 2^{H(\eps) p}$ for $p\geq 1$, $0 \leq \eps \leq \frac{1}{2}$, where $H(\eps)=-\eps \lg \eps - (1-\eps)\lg(1-\eps) \leq 2\eps \lg \frac{1}{\eps}$. 
For $\eps=\frac{1}{\Delta\alpha+1}$ we have:

$$\lg \left(2^m\binom{(\Delta\alpha+1)m}{m}\right) < m + (\Delta\alpha+1)m \cdot 2\eps \lg\frac{1}{\eps} = \left(1 + 2 \lg(\Delta \alpha+1)\right)m.$$

Hence it remains to show that $1 + 2 \lg(\Delta \alpha+1) \leq \alpha$.
Indeed $1 + 2 \lg(\Delta \alpha+1) \leq 2 \lg(2\Delta \alpha + 2\alpha)  \leq 2 \lg(\Delta + 1) + 2 \lg (2\alpha) $, which is $\leq \alpha$ for $\alpha = c \lceil \log (\Delta+1)\rceil$ and $c$ a large enough constant.
\cqed
\end{proof}

Therefore a vector with minimal support cannot have $|\supp(\vex)|\geq 2h = \Theta(m\log \Delta)$.
\end{proof}
